Global existence of weak solutions of a model for electrolyte solutions - Part 1: Two-component case

This paper analytically investigates the Darcy-Poisson-Nernst-Planck system. This system is a mathematical model for electrolyte solutions. In this paper, we consider electrolyte solutions, which consist of a neutral fluid and two suspended oppositely charged chemical species with arbitrary valencies z_1 > 0 > z_2. We prove global existence and uniqueness of weak solutions in two space dimensions and three space dimensions. So far, most of the existence results have been proven for symmetric electrolyte solutions. These solutions consist of a neutral fluid and two suspended charged chemical species with symmetric valencies +/-z. As many electrolyte solutions in biological applications and hydrodynamical applications are not symmetric, the presented extension of the previous existence results is an important step.

==> Paper2ComponentArXiv/macros_herz.tex <==
%===========================================================================================
%===========================================================================================
%
%  I   GLOBAL MATHEMATICAL MACROS 
%
%===========================================================================================
%===========================================================================================
\usepackage{xargs}   %usepackage for macros with several default parameters
%==================================================
%  I.0  Symbols 
%==================================================
% \renewcommand{\endproof}{\square}
%==================================================
%  I.1  Names
%==================================================
\newcommand{\Avogadro}{Avogadro}
\newcommand{\GagNirenberg}{Gagliardo-Nirenberg's inequality}
\newcommand{\Gronwall}{Gronwall's inequality}       % correct spelling
\newcommand{\Grownwall}{Gronwall's inequality}      % catch misspelling
\newcommand{\Holder}{H\"{o}lder's inequality}
\newcommand{\Lifshitz}{Lifshitz}
\newcommand{\Poincare}{Poincar\'{e}'s inequality}
\newcommand{\stekav}{Steklov average}
\newcommand{\vdW}{van der Waals}
\newcommand{\Young}{Young's inequality}
\newcommand*{\dnpp}{Darcy-Poisson-Nernst-Planck system}
\newcommand*{\snpp}{Stokes-Poisson-Nernst-Planck system}
%word macros for constistent writing 
%\newcommand{\theorem}{\ensuremath{ \textnormal{Theorem} }}
%\newcommand{\Lemma}{Lemma}
%\newcommand{\Definition}{Definition}
%==================================================
%   I.2  Mathematical terms
%==================================================
\newcommand{\diam}[1]{\ensuremath{ \textnormal{diam}\left( {#1} \right) }}  % \diam{x}
\newcommand{\dist}[1]{\ensuremath{ \textnormal{dist} \left( {#1} \right) }} % \dist{x} 
\newcommand{\Div}{\ensuremath{ \textnormal{div} }}                          % \Div
\newcommand{\Heavi}{\ensuremath{ \textnormal{H} }}                          % \Heavi
\newcommand{\loc}{\ensuremath{ \textnormal{loc} }}                          % \loc
\newcommand{\mol}{\ensuremath{ \textit{mol} }}                              % \mol    
\newcommand{\osc}[1]{\ensuremath{ \textnormal{osc}\left( {#1} \right) }}    % \osc{x} 
\newcommand{\Sign}{\ensuremath{ \textnormal{sign} }}                         % \Sign
\newcommand{\sign}[1]{\ensuremath{ \epsilon\left( {#1} \right) }}           % \sign{x}
\newcommand{\spt}[1]{\ensuremath{ \textnormal{spt}\left( {#1} \right) }}    % \spt{x}
\newcommand{\trace}[1]{\ensuremath{ \textnormal{tr}\left( {#1} \right) }}   % \trace{x}
\newcommand{\weak}{\ensuremath{ \textnormal{weak} }}                        % \weak
\newcommand{\weakstar}{ \textnormal{weak}^\ast }                            % \weakstar
\newcommand{\WLOG}{\ensuremath{ \textnormal{w.l.o.g.} }}                    % \wlog    
\newcommand{\esssup}{\ensuremath{ \textnormal{esssup} }}                    % \esssup                                               
%%==================================================
%  I.3  Greek Letters
%==================================================
%capture misspelling
\newcommand{\lamdba}{\ensuremath{ \lambda }}
%shortcuts             
\newcommand{\vphi}{\ensuremath{ \varphi }}                      
\newcommand{\veps}{\ensuremath{ \varepsilon }}
\newcommand{\eps}{\ensuremath{ \epsilon }}
%==================================================
%  I.4.1 Set of Numbers
%==================================================
\newcommand{\setN}{\ensuremath{ \mathbb{N} }}                   
\newcommand{\setZ}{\ensuremath{ \mathbb{Z} }}                   
\newcommand{\setR}{\ensuremath{ \mathbb{R} }}                   
\newcommand{\setC}{\ensuremath{ \mathbb{C} }}                                                               
%==================================================
%  I.4.2  Frequently used sets
%==================================================
\newcommand*{\OmegaT}[1][T]{\ensuremath{ \Omega_{#1} }}      % parabolic cylinder: \OmegaT[x] 
\newcommand*{\GammaT}[1][T]{\ensuremath{ \Gamma_{#1} }}      % parabolic boundary: \GammaT[x]
\newcommand*{\Omegad}{\ensuremath{ \OmegaT[h] }}             % discrete domain: \Omegad[x] 
\newcommand*{\Gammad}{\ensuremath{ \GammaT[h] }}             % discrete boundary: \Gammad[x]
\newcommand*{\mesh}[1][h]{\ensuremath{ \mathcal{T}_{#1} }}   % triangulation: \mesh[x] 
\newcommand*{\meshEl}{\ensuremath{ K_h }}                    % triangulation element: \TriangEl 
%==================================================
%  I.5  Brackets and arrows and relations
%==================================================
%brackets
\newcommand*{\brac}[1]{\ensuremath{ \left( {#1} \right) }}                       % bracket: \brac{xx}                     
\newcommand*{\sqbrac}[1]{\ensuremath{ \left[ {#1} \right] }}                     % squared bracket: \sqbrac{xx}                     
\newcommand*{\cbrac}[1]{\ensuremath{ \left\{ {#1} \right\} }}                    % curly bracket \cbrac{xx}                       
%arrows
\newcommand*{\hence}{\ensuremath{ ~~\Rightarrow~~ }}                             % implication arrow with more spacing
\newcommand*{\Hence}{\ensuremath{ ~~\Longrightarrow~~ }}                         % long implication arrow with more spacing
\newcommand*{\equivalent}{\ensuremath{ ~~\Leftrightarrow~~ }}                    % equivalence arrow with more spacing                                                                                                                         
\newcommand*{\Equivalent}{\ensuremath{ ~~\Longleftrightarrow~~ }}                % long equivalence arrow with more spacing   
\newcommand*{\convStrong}{\ensuremath{ ~\rightarrow~ }}                          % arrow for norm convergence                                      
\newcommand*{\ConvStrong}{\ensuremath{ ~\longrightarrow~ }}                      % long arrow for norm convergence     
\newcommand*{\convWeak}{\ensuremath{ ~\rightharpoonup~ }}                        % arrow for weak convergence                                                
\newcommand*{\convWeakstar}{\ensuremath{ \stackrel{\ast}{\,\,\rightharpoonup} }} % arrow for weakstar convergence    
%relations
\DeclareMathOperator*{\nequiv}{\textbf{/}\!\!\!\!\!\!\equiv}        
%==================================================
%  I.6.1  Vectors and Norms for Vectors
%==================================================
\renewcommand*{\vec}[1]{ \ensuremath{ \boldsymbol{#1} }}  % Vector: \vec{x}
\newcommand*{\abs}[1]{\left| {#1} \right| }               % Vectornorm: \abs{x} 
\newcommand*{\absE}[1]{\left| {#1} \right|_2 }            % Vectornorm: Eucledian norm
\newcommand*{\absF}[1]{\left| {#1} \right|_F }            %Vectornorm: Forbenius norm
%==================================================
%  I.6.2  Shortcuts for frequently used vectors
%================================================== 
\newcommand*{\vecone}{\vec{1}}
\newcommand*{\veca}{\vec{a}}
\newcommand*{\vecA}{\vec{A}}
\newcommand*{\vecb}{\vec{b}}
\newcommand*{\vecbeta}{\vec{\beta}}
\newcommand*{\vecB}{\vec{B}}
\newcommand*{\vecc}{\vec{c}}
\newcommand*{\vecD}{\vec{D}}
\newcommand*{\vece}{\vec{e}}
\newcommand*{\vecE}{\vec{E}}
\newcommand*{\vecF}{\vec{F}}
\newcommand*{\vecg}{\vec{g}}
\newcommand*{\vecH}{\vec{H}}
\newcommand*{\vecf}{\vec{f}}
\newcommand*{\veci}{\vec{i}}
\newcommand*{\vecj}{\vec{j}}
\newcommand*{\vecJ}{\vec{J}}
\newcommand*{\vecK}{\vec{K}}
\newcommand*{\vecn}{\vec{n}}
\newcommand*{\vecnu}{\vec{\nu}}
\newcommand*{\vecnull}{\vec{0}}
\newcommand*{\vecP}{\vec{P}}
\newcommand*{\vecq}{\vec{q}}
\newcommand*{\vecr}{\vec{r}}
\newcommand*{\vecrho}{\vec{\rho}}
\newcommand*{\vecS}{\vec{S}}
\newcommand*{\vecsigma}{\vec{\sigma}}
\newcommand*{\vect}{\vec{t}}
\newcommand*{\vecT}{\vec{T}}
\newcommand*{\vectau}{\vec{\tau}}
\newcommand*{\vecu}{\vec{u}}
\newcommand*{\vecv}{\vec{v}}
\newcommand*{\vecV}{\vec{V}}
\newcommand*{\vecw}{\vec{w}}
\newcommand*{\vecx}{\vec{x}}
\newcommand*{\vecz}{\vec{z}}
%==================================================
%  I.7  Products on Banach spaces        
%==================================================   
\newcommand*{\scp}[3][~]{\ensuremath{ \left( {#2}{#1},{#1}{#3} \right) }}    % scalar product:  \scp[spacing]{x}{y} 
\newcommand*{\dualp}[3][~]{\ensuremath{ \left\langle {#2}{#1},{#1}{#3} \right\rangle }} % dual pairing:   \dualp[spacing]{x}{y}        
%==================================================
%  I.8  Dervivatives
%==================================================
\renewcommand*{\grad}{\vec{\nabla}\!}                       % gradient: \grad 
\newcommand*{\dtot}{ \textnormal{d}}                      % differential: \dtot 
\newcommand*{\derd}[1][i]{\ensuremath{ \partial_{{#1}} }} % directional derivative: \derd[opt]
\newcommand*{\dert}[1][t]{\ensuremath{ \partial_{{#1}} }} % temporal derivative: \dert[opt]   
\newcommand*{\derm}[1][t]{\ensuremath{ \frac{D}{D{#1}} }} % material derivative: \derm[opt]
\newcommand*{\derr}[1][t]{\ensuremath{ \frac{d}{d{#1}} }} % dervative on real line: \derr[opt]
%==================================================
%  I.9  Integrals
%==================================================
\newcommand{\Int}[4]{\ensuremath{ \int\limits_{#2}^{{#3}} {#4} d{#1} }}    % Integral:   \Int{integrand variable}{subscript}{superscript}{function}  
\newcommand*{\Intdx}[2][\Omega]{ \Int{x}{{#1}}{}{{#2}} }                   % Volume integral with respect to dx and defaluft domain: \Intdx[domain]{function}
\newcommand*{\IntdS}[2][\Gamma]{ \Int{S}{{#1}}{}{{#2}} }                   % Surface integral with respect to dS and default domain: \IntdS[domain]{function}           
\newcommandx*{\Intdt}[3][1=0,2=T,usedefault]{ \Int{t}{{#1}}{{#2}}{{#3}} }  % Time integral with respect to dt and default interval:  \Intdt[lower border][upper border]{function}
%======================================================
%  I.10  Function Spaces and Norms of Function Spaces
%======================================================
\newcommandx*{\fspace}[4][1=-1pt,usedefault]{ \ensuremath{  {{#2}} \hspace{#1} \left( {#3}{#4} \right) }} % Function space: \fspace[hspace]{name}{domain}{range} 
\newcommandx*{\norm}[2]{ \ensuremath{ \left\| {#1} \right\|_{{#2}}   }}                                   % Norms for functions: \norm{object}{space} 
%========================================
%  I.10.1   Ck Spaces        
%========================================       
\newcommandx*{\Ck}[4][1=\Omega,2= ,usedefault]{ \fspace{ C^{{#3}}_{{#2}} }{ {#1} }{ {#4} } } %\Ck[domain][subscript]{smoothness k}{range}  
%========================================
%  I.10.2   Lp Spaces        
%========================================       
\newcommandx*{\Lp}[4][1=\Omega,2= ,usedefault]{ \fspace{ L^{{#3}}_{{#2}} }{ {#1} }{ {#4} } } %\Lpk[domain][subscript]{exponent p}{range} 
%========================================
%  I.10.3  Sobolev Spaces        
%========================================
\newcommandx*{\Wkp}[5][1=\Omega,2= ,usedefault]{ \fspace{ W^{{#3},{#4}}_{{#2}} }{ {#1} }{ {#5} } } % \Wkp[domain][subscript]{smoothness k}{exponent p}{range}                
\newcommandx*{\Hk}[4][1=\Omega,2= ,usedefault]{ \fspace{ H^{{#3}}_{{#2}} }{ {#1} }{ {#4} } }       % \Hk[domain][subscript]{smoothness k}{range}                      
\newcommandx*{\Hkdiv}[3][1=\Omega,2= ,usedefault]{ \fspace{ H^{{#3}}_{{#2}} }{\Div}{;{#1}} }       % \Hkdiv[domain][subscript]{smoothness k}
%
%
%===========================================================================================
%===========================================================================================
%
%  II   MATHEMATICAL MACROS FOR CURRENT PAPER
%
%===========================================================================================
%===========================================================================================
\usepackage{xargs}   %usepackage for macros with several default parameters 
%=====================================================================
%  II.1  Shortcuts for frequently used continuous spaces
%=====================================================================  
\newcommand{\spaceTC}{ \Hk{1}{} }                                                         % Concentrations: Test function space
\newcommand{\spaceSC}{ \fspace{L^2}{I}{; \Hk{1}{} } \cap \fspace{H^1}{I}{; \Hk{1}{}^* } } % Concentrations: Solution space
\newcommand{\spaceTF}{ \Hkdiv[][0]{} }                                                    % Velocity: Test function space
\newcommand{\spaceSF}{ \fspace{L^\infty}{I}{; \Hkdiv[][f]{} } }                           % Velocity: Solution space
\newcommand{\spaceTP}{ \Lp{2}{} }                                                         % Pressure: Test function space
\newcommand{\spaceSP}{ \fspace{L^\infty}{I}{; \Lp{2}{}/\setR } }                          % Pressure: Solution space
\newcommand{\spaceTEF}{ \Hkdiv[][0]{} }                                                   % Electrostatic Potential: Test function space
\newcommand{\spaceSEF}{ \fspace{L^\infty}{I}{; \Hkdiv[][\sigma]{} }  }                    % Electrostatic Potential: Solution space
%==================================================
%  II.2  Variables of the continuous system
%==================================================
\newcommand*{\tx}{(t,x)}    % continuous variables (t,x)
\newcommand*{\timeEnd}{T_0} % end time T_0

\newcommand*{\test}{\ensuremath{ \vphi }} % Test function: scalar
\newcommand*{\Test}{\ensuremath{ \vecv }} % Test function: vector

\newcommand*{\boltz}{\ensuremath{ k_b }}                                                 % Parameters: Boltzmann Constant
\newcommand*{\temp}{\ensuremath{ T }}                                                    % Parameters: Temperature
\newcommand*{\thermEnergy}{\ensuremath{ \boltz\temp }}                                   % Parameters: thermal energy
\newcommand*{\Dl}[1][]{\ensuremath{ D_{{#1}} }}                                          % Parameters: Diffusion coefficient
\newcommand*{\zl}[1][l]{\ensuremath{ z_{{#1}} }}                                         % Parameters: Valency
\newcommand*{\mob}[1][]{\ensuremath{ \omega_{{#1}} }}                                    % Parameters: Mobility
\newcommand*{\wl}[1][l]{\ensuremath{ e\zl[{#1}]\mob }}                                   % Parameters: Electrophoretic mobility
\newcommand*{\permitELscalar}{\ensuremath{ \epsilon }}                                   % Parameters: Electric permittivity constant
\newcommand*{\permitEL}{\ensuremath{ \mathcal{E} }}                                      % Parameters: Electric permittivity tensor
\newcommand*{\permeabH}{\ensuremath{ K }}                                                % Parameters: Hydraulic permeability
\newcommand*{\viscos}{\ensuremath{ \mu }}                                                % Parameters: dynamic viscosity
\newcommand*{\coeffEL}[1][l]{\ensuremath{e\zl[{#1}](\permitELscalar\boltz\temp)^{-1} }}  % Parameters: Electric coefficient in Transport
\newcommand*{\coeffForceEL}{\ensuremath{\mu^{-1}\permitEL^{-1}}}

\newcommand{\cl}[1][l]{\ensuremath{ c_{{#1}} }}                  % Concentrations: l-th concentration
\newcommand{\Cl}{\ensuremath{ \vecc }}                           % Concentrations: vector
\newcommand{\clstart}[1][l]{\ensuremath{ c_{0,{#1}} }}           % Concentrations: Initial value for l-th concentration
\newcommand{\Clstart}{\ensuremath{\vecc_{0} }}                   % Concentrations: Initial value vector
\newcommand{\gl}[1][l]{ g_{{#1}} }                               % Concentrations: boundary flux of l-th concentration
\newcommand{\Gl}{ \vecg }                                        % Concentrations: boundary flux vector
\newcommand{\clflux}[1][l]{\ensuremath{ \vecj_{{#1}} }}          % Concentrations: mass flux of l-th concentration
\newcommand{\clcharge}[1][l]{\ensuremath{ e\zl[{#1}]\cl[{#1}] }} % Concentrations: charge of l-th concentration                                                                        
\newcommand{\Rl}[1][l]{\ensuremath{ R_{{#1}} }}                                 % Reactions: reaction rate in equation for l-th concentration   
\newcommand{\Rlfunc}[1][c]{\ensuremath{\Rl\left({#1}_1,\ldots,{#1}_L \right) }} % Reactions: reaction rate with arguments in equation for l-th concentration 


\newcommand{\fieldF}{\ensuremath{ \vecu }} % Velocity: Flow field
\newcommand{\press}{p}                     % Pressure: Pressure field

\newcommand{\potEL}{\ensuremath{ \Phi }}                                    % Electrostatic:  Electric Potential
\newcommand{\fieldEL}{\ensuremath{ \vecE }}                                 % Electrostatic:  Electric field
\newcommand*{\chargeEL}[1][]{ \ensuremath{ \rho_{f{#1}} } }                 % Electrostatic:  Free charge density -- short
\newcommand*{\chargeELlong}[1][l]{ \sum_l\zl\cl }                           % Electrostatic:  Free charge density -- long
\newcommand*{\chargeELlongTwo}[1][l]{ \zl[1]\cl[1]-\abs{\zl[2]}\cl[2] }     % Electrostatic:  Free charge density 2 species -- long
\newcommand*{\forceEL}[1][]{\ensuremath{ \chargeEL[{#1}] \fieldEL_{{#1}} }} % Electrostatic:  Electroosmotic force -- short
%==================================================
%  II.2  Modified Concentrations
%==================================================
\newcommand{\clk}[1][l]{\ensuremath{ (c_{{#1}}-k)_+ }}    % Lower Truncated Concentrations: l-th concentration
\newcommand{\Clk}{\ensuremath{ (\vecc-k\vecone) }}        % Lower Truncated Concentrations: vector
\newcommand{\clm}[1][l]{\ensuremath{ c_{{#1}}^m }}        % Upper Truncated Concentrations: l-th concentration
\newcommand{\Clm}{\ensuremath{ \vecc^m }}                 % Upper Truncated Concentrations: vector
\newcommand{\clkm}[1][l]{\ensuremath{ (c^m_{{#1}}-k)_+ }} % Lower and Upper Truncated Concentrations: l-th concentration
\newcommand{\Clkm}{\ensuremath{ (\vecc^m-k\vecone) }}     % Lower and Upper Truncated Concentrations: vector
%==================================================
%  II.3  Fixed Point Approach
%==================================================
\newcommand{\fixOp}{\ensuremath{\mathcal{F}}}
\newcommand{\fixSet}{\ensuremath{K}}
\newcommand{\fixSpace}{\ensuremath{X}}

\newcommand{\clold}[1][l]{\ensuremath{\bar{c}_{{#1}} }}                           % Old Concentrations
\newcommand{\Clold}{\ensuremath{ \bar{\vecc} }}                                   % Old Concentration vector
\newcommand*{\chargeELold}[1][]{ \ensuremath{ \bar{\rho}_{f{#1}} } }              % Old free charge density -- short
\newcommand*{\chargeELlongold}[1][l]{ \sum_l\zl\clold }                           % Old free charge density -- long
\newcommand*{\chargeELlongTwoold}[1][l]{ \zl[1]\clold[1]-\abs{\zl[2]}\clold[2] }  % Old free charge density 2 species -- long
\newcommand*{\forceELold}[1][]{\ensuremath{ \chargeELold[{#1}] \fieldEL_{{#1}} }} % Old electroosmotic force -- short
%==================================================
%  II.4  Entropy Methods
%==================================================
\newcommand{\lyapunov}{\Lambda}

==> Paper2ComponentArXiv/thm-environments-report.tex <==
% 1. uncomment for standard theorem environments 
\usepackage{amsthm}         % math theorem environments

% 2. uncomment for framed theorem environments with ntheorem: option amsthm for compatibility with amsthm. comment amsthm above 
%\usepackage[amsmath,framed,thmmarks,amsthm]{ntheorem}  

% 3. uncomment for framed theorem environments with mdframed 
\usepackage[framemethod=PSTricks]{mdframed}        



% 1. standard theorem environments 
%
% 1.1 theorem environments with italic letters 
\theoremstyle{plain}    
   %Theorem
   \crefformat{thm}{Theorem~#2#1#3}                %define citation format for counter "thm"
   \newtheorem{thm}{Theorem}[chapter]              %define new environment "thm" that automatically creates a counter "thm". Choose numbering subordinate to chapters    
   \crefname{thm}{Theorem}{Theorems}               %define single/plural citation names for environment "thm"
   %Proposition    
   \crefformat{count_prop}{Proposition~#2#1#3}        %define citation format for counter "count_prop"
   \newaliascnt{count_prop}{thm}                      %define counter "count_prop" as a alias for the counter "thm". This enables consecutive numbering.
   \newtheorem{proposition}[count_prop]{Proposition}  %define new environment "proposition" that uses the counter "count_prop" with the above specified citation format 
   \aliascntresetthe{count_prop}                      %close definition
   \crefname{proposition}{Proposition}{Propositions}  %define single/plural citation names for environment "proposition"
   %Lemma 
   \crefformat{count_lem}{Lemma~#2#1#3}       
   \newaliascnt{count_lem}{thm}               
   \newtheorem{lemma}[count_lem]{Lemma}        
   \aliascntresetthe{count_lem}                
   \crefname{lemma}{Lemma}{Lemmas}
   %Definition
   \crefformat{count_defi}{Definition~#2#1#3}       
   \newaliascnt{count_defi}{thm}
   \newtheorem{definition}[count_defi]{Definition}
   \aliascntresetthe{count_defi}                
   \crefname{definition}{Definition}{Definitions}
   %Corollary
   \crefformat{count_cor}{Corollary~#2#1#3}       
   \newaliascnt{count_cor}{thm}
   \newtheorem{corollary}[count_cor]{Corollary} 
   \aliascntresetthe{count_cor}                
   \crefname{corollary}{Corollary}{Corollaries}

% 1.2 theorem environments with normal letters
\theoremstyle{definition}  
   %Remark                        
   \crefformat{count_rem}{Remark~#2#1#3}       
   \newaliascnt{count_rem}{thm}
   \newtheorem{remark}[count_rem]{Remark}
   \aliascntresetthe{count_rem}                
   \crefname{remark}{Remark}{Remarks}
    %Example
   \crefformat{count_exmpl}{Example~#2#1#3}       
   \newaliascnt{count_exmpl}{thm}
   \newtheorem{example}[count_exmpl]{Example}
   \aliascntresetthe{count_exmpl}                
   \crefname{example}{Example}{Examples}



% 2. framed theorem environments with ntheorem: 
%
% 2.1 framed theorem environments with italic letters 
%\theoremstyle{plain}  
%    \newframedtheorem{fthm}{Theorem}[section]             %[section]: numbering subordinate to chapters                  
%    \newframedtheorem{fproposition}[fthm]{Proposition}    %[fthm]: use fthm counter    
%    \newframedtheorem{flemma}[fthm]{Lemma}                %[fthm]: use fthm counter
%    \newframedtheorem{fdefinition}[fthm]{Definition}      %[fthm]: use fthm counter
%    \newframedtheorem{fcorollary}[fthm]{Corollary}        %[fthm]: use fthm counter
%
% 2.2 framed theorem environments with normal letters
%\theoremstyle{definition} 
%    \newframedtheorem{fremark}[fthm]{Remark}              %[fthm]: use fthm counter



   
% 3. framed environments with mdframed
%
% 3.1 framed theorem environments with italic letters
   %Theorem
   \crefformat{fthm}{Theorem~#2#1#3}               %define citation format for counter "fthm"
   \mdtheorem{fthm}{Theorem}[section]              %define new environment "fthm" that automatically creates a counter "fthm". Choose numbering subordinate to chapters    
   \crefname{fthm}{Theorem}{Theorems}              %define single/plural citation names for environment "thm"
   %Proposition
   \crefformat{count_fprop}{Proposition~#2#1#3}        %define citation format for counter "count_fprop"
   \newaliascnt{count_fprop}{fthm}                     %define counter "count_fprop" as a alias for the counter "fthm". This enables consecutive numbering.
   \mdtheorem{fproposition}[count_fprop]{Proposition}  %define new environment "fproposition" that uses the counter "count_fprop" with the above specified ciation format 
   \aliascntresetthe{count_fprop}                      %close definition
   \crefname{fproposition}{Proposition}{Propositions}  %define single/plural citation names for environment "fproposition"
   %Lemma
   \crefformat{count_flem}{Lemma~#2#1#3} 
   \newaliascnt{count_flem}{fthm}
   \mdtheorem{flemma}[count_flem]{Lemma}                
   \aliascntresetthe{count_flem}
   \crefname{flemma}{Lemma}{Lemmas}
   %Definition  
   \crefformat{count_fdefi}{Definition~#2#1#3}
   \newaliascnt{count_fdefi}{fthm}
   \mdtheorem{fdefinition}[count_fdefi]{Definition}      
   \aliascntresetthe{count_fdefi}
   \crefname{fdefinition}{Definition}{Definitions}
   %Corollary
   \crefformat{count_fcor}{Corollary~#2#1#3}
   \newaliascnt{count_fcor}{fthm}
   \mdtheorem{fcorollary}[count_fcor]{Corollary}       
   \aliascntresetthe{count_fcor}
   \crefname{fcorollary}{Corollary}{Corollary}
   %Remark 
   \crefformat{count_frem}{Remark~#2#1#3}
   \newaliascnt{count_frem}{fthm}
   \mdtheorem{fremark}[count_frem]{Remark}
   \aliascntresetthe{count_frem}
   \crefname{fremark}{Remark}{Remarks}
    %Example
   \crefformat{count_fexmpl}{Example~#2#1#3}       
   \newaliascnt{count_fexmpl}{thm}
   \mdtheorem{fexample}[count_fexmpl]{Example}
   \aliascntresetthe{count_fexmpl}                
   \crefname{fexample}{Example}{Examples}
      
      
   
